Self-supervised Dataset Distillation: A Good Compression Is All You Need

Dataset distillation aims to compress information from a large-scale original dataset to a new compact dataset while striving to preserve the utmost degree of the original data informational essence. Previous studies have predominantly concentrated on aligning the intermediate statistics between the original and distilled data, such as weight trajectory, features, gradient, BatchNorm, etc. In this work, we consider addressing this task through the new lens of model informativeness in the compression stage on the original dataset pretraining. We observe that with the prior state-of-the-art SRe$^2$L, as model sizes increase, it becomes increasingly challenging for supervised pretrained models to recover learned information during data synthesis, as the channel-wise mean and variance inside the model are flatting and less informative. We further notice that larger variances in BN statistics from self-supervised models enable larger loss signals to update the recovered data by gradients, enjoying more informativeness during synthesis. Building on this observation, we introduce SC-DD, a simple yet effective Self-supervised Compression framework for Dataset Distillation that facilitates diverse information compression and recovery compared to traditional supervised learning schemes, further reaps the potential of large pretrained models with enhanced capabilities. Extensive experiments are conducted on CIFAR-100, Tiny-ImageNet and ImageNet-1K datasets to demonstrate the superiority of our proposed approach. The proposed SC-DD outperforms all previous state-of-the-art supervised dataset distillation methods when employing larger models, such as SRe$^2$L, MTT, TESLA, DC, CAFE, etc., by large margins under the same recovery and post-training budgets. Code is available at https://github.com/VILA-Lab/SRe2L/tree/main/SCDD/.

==> table/BN_para.tex <==
\begin{table}[h]
\centering
\resizebox{0.65\linewidth}{!}{
\begin{tabular}{@{}cccc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Frist BN multiplier\\ recovery parameter\end{tabular}} & \multicolumn{3}{c}{validation accuracy (\%)} \\ \cmidrule(l){2-4} 
         & ResNet-18 & ResNet-50 & ResNet-101 \\ \midrule
1$\times$       &  52.49   &  60.10    & 58.98   \\
5$\times$       &  53.09   &  60.43    & \bf 61.11  \\
10$\times$      &  \bf 53.13   & \bf 60.92    &  60.98    \\
15$\times$      &  50.96   &  58.15    & 56.29  \\
20$\times$      &  50.82   &  57.69   &  57.30  \\ \bottomrule
\end{tabular}
}
\caption{Ablation on the coefficient of the frist BN loss term in Eq.~\ref{BN_coefficient} when $k=0$, other layers' coefficients are set to 1 following~\cite{yin2023squeeze}. We presnet validation results on distilled data with IPC 50 recovered from MoCo-v3-300ep ResNet-50 in recovery phase.} 
\label{tab:BN_para}
\vspace{-0.1in}
\end{table}


==> table/IPC200.tex <==
\begin{table}[h]
\centering
\begin{tabular}{@{}cccc@{}}
\toprule
\multicolumn{2}{c}{Validation Accuracy} \\ \midrule
  SRe$^2$L & Ours \\ \midrule
  64.6$\pm$0.3  &  68.45$\pm$0.1  \\
\bottomrule
\end{tabular}
\caption{Validation accuracy on recovery IPC 200 comparing SRe$^2$L and our method.}
\label{tab:IPC200}
\end{table}



==> table/baseline.tex <==
\begin{table}[]
\begin{tabular}{@{}cccc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}SRe$^2$L\\ recovery model\end{tabular}} & \multicolumn{3}{c}{validation accuracy} \\ \cmidrule(l){2-4} 
           & ResNet-18 & ResNet-50 & ResNet-101 \\ \midrule
ResNet-18  &  43.690   &  48.358   &  51.566 \\
ResNet-50  &  40.660   &  46.016   &  49.060\\
ResNet-101 &  39.950   &  45.564   &  48.924\\ \bottomrule
\end{tabular}
\caption{Validation results on distilled datasets recovered from different-scale ResNet models.}
\label{tab:baseline}
\end{table}


==> table/cifar100.tex <==
\begin{table}[]
\begin{tabular}{@{}cccc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}CIFAR-100\\ recovery model\end{tabular}} & \multicolumn{3}{c}{validation accuracy} \\ \cmidrule(l){2-4} 
           & ResNet-18  & ResNet-50  & ResNet-101 \\ \midrule
ResNet-18  &   56.625   &  58.667    &   58.000  \\
ResNet-50  &   53.333   &   55.667   &   54.333 \\ \bottomrule
\end{tabular}
\caption{Validation results on distilled datasets recovered from different-scale MoCo v2 models based on CIFAR-100 dataset.}
\label{tab:cifar100_model}
\end{table}


==> table/config_IM_pretrain.tex <==
\begin{table}[]
\begin{tabular}{l|l}
Config             & Value    \\ \midrule
optimizer          &  SGD            \\
base learning rate &  20.0   \\
weight decay       &   0.0  \\
optimizer momentum &  0.9  \\
batch size         &  512 \\
learning rate schedule & cosine decay  \\
\end{tabular}
\label{tab:config_IM_pretrain}
\caption{Pretrain MoCo v3 based on Resnet50.}
\end{table}



==> table/config_IM_recover.tex <==
\begin{table}[]
\begin{tabular}{l|l}
Config             & Value    \\ \midrule
$\alpha_{BN}$      &  0.25            \\
optimizer          &  AdamW            \\
base learning rate &  0.35   \\
weight decay       &     \\
optimizer momentum &    \\
batch size         &  50 \\
learning rate schedule & cosine decay  \\
recovering iteration & 1000 \\
augmentation       &   RandomResizedCrop  \\
\end{tabular}
\label{tab:config_IM_recover}
\caption{ImageNet-1K recovering setting.}
\end{table}

==> table/config_IM_validation.tex <==
\begin{table}[]
\begin{tabular}{l|l}
Config             & Value    \\ \midrule
optimizer          &  AdamW            \\
base learning rate &  0.001   \\
weight decay       &  0.01   \\
batch size         &  64 \\
learning rate schedule &  cosine decay \\
training epoch & 300 \\
augmentation       &  RandomResizedCrop   \\
\end{tabular}
\label{tab:config_IM_validation}
\caption{ImageNet-1K validation setting.}
\end{table}

==> table/config_cifar_pretrain.tex <==
\begin{table}[]
\begin{tabular}{l|l}
Config             & Value    \\ \midrule
$\alpha_{BN}$      &   8     \\
optimizer          &   SGD           \\
base learning rate &   0.06 \\
weight decay       &   5e-4  \\
optimizer momentum &  0.99  \\
batch size         & 512  \\
learning rate schedule & cosine decay \\
\end{tabular}
\label{tab:config_cifar_pretrain}
\caption{Pretrain MoCo v2 ResNet50 on CIFAR-100.}
\end{table}

==> table/config_cifar_recover.tex <==
\begin{table}[]
\begin{tabular}{l|l}
Config             & Value    \\ \midrule
$\alpha_{BN}$      &    0.1    \\
optimizer          &    Adam          \\
base learning rate &  0.2  \\ 
weight decay       &     \\
optimizer momentum &       \\
batch size         & 100  \\
learning rate schedule & cosine decay  \\
recovering iteration & 300 \\
augmentation       &   RandomResizedCrop  \\
\end{tabular}
\label{tab:config_cifar_recover}
\caption{CIFAR-100 recovering setting.}
\end{table}

==> table/config_cifar_validation.tex <==
\begin{table}[]
\begin{tabular}{l|l}
Config             & Value    \\ \midrule
optimizer          &   AdamW           \\
base learning rate &   0.1  \\
weight decay       &  1e-4   \\
optimizer momentum &   0.9 \\
batch size         &  128 \\
learning rate schedule & CosineAnnealingLR  \\
training epoch & 1000 \\
\end{tabular}
\label{tab:config_cifar_squeeze}
\caption{CIFAR-100 validation setting.}
\end{table}

==> table/config_tiny_pretrain.tex <==
\begin{table}[]
\begin{tabular}{l|l}
Config             & Value    \\ \midrule
$\alpha_{BN}$      &   8     \\
optimizer          &   SGD           \\
base learning rate &   0.06 \\
weight decay       &   5e-4  \\
optimizer momentum &  0.99  \\
batch size         & 512  \\
learning rate schedule & cosine decay \\
\end{tabular}
\label{tab:config_tiny_pretrain}
\caption{Pretrain MoCo v2 ResNet50 on Tiny-ImageNet.}
\end{table}

==> table/config_tiny_recover.tex <==
\begin{table}[]
\begin{tabular}{l|l}
Config             & Value    \\ \midrule
$\alpha_{BN}$      &   0.1     \\
optimizer          &   Adam           \\
base learning rate &   0.5  \\ 
weight decay       &     \\
optimizer momentum &       \\
batch size         &  100 \\
learning rate schedule &  cosine decay \\
recovering iteration & 1000 \\
augmentation       &  RandomResizedCrop   \\
\end{tabular}
\label{tab:config_tiny_recover}
\caption{Tiny-ImageNet recovering setting.}
\end{table}

==> table/config_tiny_validation.tex <==
\begin{table}[]
\begin{tabular}{l|l}
Config             & Value    \\ \midrule
optimizer          &   SGD           \\
base learning rate &   0.35  \\
weight decay       &  1e-4   \\
optimizer momentum &   0.9 \\
batch size         &  96 \\
learning rate schedule & cosine decay  \\
training epoch & 1000 \\
augmentation       &   RandomResizedCrop  \\
\end{tabular}
\label{tab:config_tiny_squeeze}
\caption{Tiny-ImageNet validation setting.}
\end{table}

==> table/cross_architecture.tex <==

\begin{table*}[t]
\centering
\resizebox{0.999\linewidth}{!}{
\begin{tabular}{@{}cccccccccc@{}}
\toprule
\multicolumn{10}{c}{Various Architectures Validation Accuracy (\%)}   \\ \midrule
  ResNet-18  & ResNet-50 & ResNet-101 & RegNet-X-8gf  & SqueezeNetV1.0  & MobileNet-V3-L & EfficientNetV2-L & MNASNet-0.5 & ShuffleNetV2-0.5x  & ViT-Tiny \\
  11.7M      & 25.6M     & 44.5M      & 39.6M         & 1.2M & 5.4M  &  121M & 2.2M & 1.4M &  5.7M \\
  53.13     & 60.92    & 60.98     & 61.94        & 22.25   &   51.65    &   58.30      &  36.93 & 27.48   & 54.13 \\ 
\bottomrule
\end{tabular}
} 
% \vspace{-0.1in}
\caption{Top-1 validation accuracy results with vaious validation models. Recovery model is pretrained using MoCo v3.}
\label{tab:cross_architecture}
\vspace{-0.15in}
\end{table*}


==> table/dino_ep.tex <==
\begin{table}[h]
\centering
\begin{tabular}{@{}cccc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}DINO\\ pretrain epoch\end{tabular}} & \multicolumn{3}{c}{validation accuracy} \\ \cmidrule(l){2-4} 
        & ResNet-18 & ResNet-50 & ResNet-101 \\ \midrule
100 &  46.080   &  55.324   &  55.412   \\
800 & 47.272    & 51.726    & 54.404     \\ \bottomrule
\end{tabular}
\caption{Validation results on distilled datasets recovered from DINO Resnet-50 with various pretrained epochs.}
\label{tab:dino_ep}
\end{table}




==> table/ipc.tex <==
\begin{table}[h]
\centering
\begin{tabular}{@{}cccc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}MoCo v3\\ recovery IPC\end{tabular}} & \multicolumn{3}{c}{validation accuracy} \\ \cmidrule(l){2-4} 
        & ResNet-18 & ResNet-50 & ResNet-101 \\ \midrule
50    &  61.180     & 66.588       &      \\
100 &  &  &  \\
150 &  &  &  \\
200 &  &  &  \\ \bottomrule
\end{tabular}
\caption{Validation results on distilled datasets recovered from MoCo v3 with pretrained epoch 300 and pretrained model ResNet50 and recovery iteration 3K.  Various recovery IPC number. Post training in 1000 epoch.}
\label{tab:ipc}
\end{table}


==> table/mix.tex <==
\begin{table}[h]
\centering
\begin{tabular}{@{}ccccc@{}} 
\toprule
Method                   & Epoch & RN-18 & RN-50 & RN-101 \\ \midrule
\multirow{4}{*}{MoCo-v2} & 100   & 45.622   &  54.878   &  51.358\\
                         & 200   &  46.624   &  56.722   &  56.596  \\
                         & 400   &  45.506   &  55.120   &  55.930   \\
                         & 800   &  39.346  & 49.926    &  50.282 \\ \midrule
\multirow{3}{*}{MoCo-v3} & 100   & 49.752       & 57.948       & 57.242     \\
                        &300   & 51.358       & 59.634       & 60.062     \\
                        &1000 & 50.622 & 59.208       & 59.226    \\ \midrule
\multirow{4}{*}{SwAV}    & 100 &  34.716   &   44.958  &   44.238   \\
                        & 200 &   47.554  &   57.320  &  56.262    \\
                        & 400 &   48.020  &   58.250  &  57.896    \\
                        & 800 & 49.700    & 58.704    & 56.386  \\ \midrule
\multirow{2}{*}{DINO}   &100 &  46.080   &  55.324   &  55.412   \\
                        &800 & 47.272    & 51.726    & 54.404   \\ \bottomrule
\end{tabular}
\caption{}
\label{tab:mix}
\end{table}



==> table/moco_v2_in21k.tex <==
\begin{table}[h]
\centering
\begin{tabular}{@{}cccc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}MoCo v2 \\in21k\end{tabular}} & \multicolumn{3}{c}{validation accuracy} \\ \cmidrule(l){2-4} 
          & ResNet-18 & ResNet-50 & ResNet-101 \\ \midrule
ResNet-18 & 40.550    & 50.34    & 48.706 \\ \bottomrule
\end{tabular}
\caption{Validation result on distilled datasets recovered from MoCo v2 models with 100 pretrain epochs.}
\label{tab:other}
\end{table}

==> table/moco_v2_model.tex <==
\begin{table}[h]
\centering
\resizebox{0.55\linewidth}{!}{
\begin{tabular}{@{}ccccc@{}}
\toprule
\multicolumn{2}{c}{\multirow{2}{*}{pretrain model}} & \multicolumn{3}{c}{validation accuracy (\%)} \\ \cline{3-5} 
\multicolumn{2}{c}{}                   & ResNet-18 & ResNet-50 & ResNet-101 \\ 
\midrule
\multirow{3}{*}{\rotatebox{90}{MoCov2}}  & ResNet-18  &  43.15 & 53.41 &  53.72 \\
 & ResNet-50  &  46.62   &  56.72   &  56.60   \\
 & ResNet-101 &   \bf  47.71 &   \bf  57.12 &   \bf   56.88 \\ 
\midrule
\multirow{4}{*}{\rotatebox{90}{SwAV}}  & ResNet-50    & 48.02  &   58.25  &  57.90 \\
 & ResNet-50-w2 &  49.80   & \bf 58.93   &  59.51  \\
 & ResNet-50-w4 & \bf 49.83   &  58.72   &  58.46     \\
 & ResNet-50-w5 &  49.59   &  58.80   & \bf 59.70    \\ \bottomrule
\end{tabular}
}
\caption{Validation results on distilled datasets recovered from MoCo v2 and SwAV with different pretrained architectures.}
\label{tab:moco_v2_model}
\vspace{-0.1in}
\end{table}


==> table/moco_v3_3K.tex <==
\begin{table}[h]
\centering
\resizebox{0.68\linewidth}{!}{
\begin{tabular}{@{}cccc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}MoCo v3 \\recovery iteration\end{tabular}} & \multicolumn{3}{c}{validation accuracy (\%)} \\ \cmidrule(l){2-4} 
& ResNet-18 & ResNet-50  & ResNet-101 \\ \midrule
1K &  51.36  & 59.78   & 60.06   \\
2K &  52.97  & 60.63   & 60.09   \\
3K & \bf 53.13  & \bf 60.92   & \bf 60.98     \\ 
4K &  51.90  & 59.98   & 60.35  \\\bottomrule
\end{tabular}
} 
\caption{Validation results on distilled datasets recovered from MoCo v3 with various recovery iterations.}
\label{tab:moco_v3_3K}
\vspace{-0.15in}
\end{table}

==> table/moco_v3_ep.tex <==
\begin{table}[h]
\centering
\begin{tabular}{@{}cccc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}MoCo v3\\ pretrain epochs\end{tabular}} & \multicolumn{3}{c}{validation accuracy} \\ \cmidrule(l){2-4} 
         & ResNet-18 & ResNet-50 & ResNet-101 \\ \midrule
100   & 49.752       & 57.948       & 57.242     \\
300   & 51.358       & 59.634       & 60.062     \\
1000 & 50.622       & 59.208       & 59.226     \\ \bottomrule
\end{tabular}
\caption{Validation results on distilled datasets recovered from MoCo v3 ResNet-50 with various pretrain epochs. }
\label{tab:moco_v3_ep}
\end{table}

==> table/swav_ep.tex <==
\begin{table}[h]
\centering
\begin{tabular}{@{}cccc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}SwAV\\ pretrain epochs\end{tabular}} & \multicolumn{3}{c}{validation accuracy} \\ \cmidrule(l){2-4} 
        & ResNet-18 & ResNet-50 & ResNet-101 \\ \midrule
100 &  34.716   &   44.958  &   44.238   \\
200 &   47.554  &   57.320  &  56.262    \\
400 &   48.020  &   58.250  &  57.896    \\
800 & 49.700    & 58.704    & 56.386      \\ \bottomrule
\end{tabular}
\caption{Validation results on distilled datasets recovered from SwAV ResNet-50 with various pretrained epochs.}
\label{tab:swav_ep}
\end{table}

==> table/swav_model.tex <==
\begin{table}[h]
\centering
\begin{tabular}{@{}cccc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}SwAV\\ recovery model\end{tabular}} & \multicolumn{3}{c}{validation accuracy} \\ \cmidrule(l){2-4} 
                      & ResNet-18 & ResNet-50 & ResNet-101 \\ \midrule
ResNet-50    & 48.020  &   58.250  &  57.896 \\
ResNet-50-w2 &  49.802   &  58.932   &  59.506  \\
ResNet-50-w4 &  49.826   &  58.718   &  58.464     \\
ResNet-50-w5 &  49.590   &  58.798   &  59.700    \\ \bottomrule
\end{tabular}
\caption{Validation results on distilled datasets recovered from  SwAV ResNet-50 variants with different architecture of pretrained models.}
\label{tab:swav_model}
\end{table}

==> table/tiny_imagenet.tex <==
\begin{table}[]
\begin{tabular}{@{}cccc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Tiny-ImageNet\\ recovery model\end{tabular}} & \multicolumn{3}{c}{validation accuracy} \\ \cmidrule(l){2-4} 
           & ResNet-18 & ResNet-50 & ResNet-101 \\ \midrule
ResNet-18  & 46.43     &  47.85    &  49.14   \\
ResNet-50  & 46.41     &  47.08    &  49.17    \\ \bottomrule
\end{tabular}
\caption{Validation results on distilled datasets recovered from different-scale MoCo v2 models based on Tiny-Imagenet. }
\label{tab:Tiny_Imagenet_model}
\end{table}

